Diffusion Probabilistic Models for Scene-Scale 3D Categorical Data

In this paper, we learn a diffusion model to generate 3D data on a scene-scale. Specifically, our model crafts a 3D scene consisting of multiple objects, while recent diffusion research has focused on a single object. To realize our goal, we represent a scene with discrete class labels, i.e., categorical distribution, to assign multiple objects into semantic categories. Thus, we extend discrete diffusion models to learn scene-scale categorical distributions. In addition, we validate that a latent diffusion model can reduce computation costs for training and deploying. To the best of our knowledge, our work is the first to apply discrete and latent diffusion for 3D categorical data on a scene-scale. We further propose to perform semantic scene completion (SSC) by learning a conditional distribution using our diffusion model, where the condition is a partial observation in a sparse point cloud. In experiments, we empirically show that our diffusion models not only generate reasonable scenes, but also perform the scene completion task better than a discriminative model. Our code and models are available at https://github.com/zoomin-lee/scene-scale-diffusion

==> content/table_tex/label_color.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|
>{\columncolor[HTML]{FFC800}}c |
>{\columncolor[HTML]{FF7832}}c |
>{\columncolor[HTML]{375A50}}c |
>{\columncolor[HTML]{FF1E1E}}c |
>{\columncolor[HTML]{FFF096}}c |}
\hline
Building & Barrier & {\color[HTML]{FFFFFF} Other} & {\color[HTML]{FFFFFF} Pedestrian} & Pole \\ \hline
\cellcolor[HTML]{FF00FF}Road & \cellcolor[HTML]{AF004B}{\color[HTML]{FFFFFF} Ground} & \cellcolor[HTML]{4B004B}{\color[HTML]{FFFFFF} Sidewalk} & \cellcolor[HTML]{00AF00}Vegetation & \cellcolor[HTML]{6496F5}Vehicles \\ \hline
\end{tabular}
\end{table}

==> content/table_tex/ours.tex <==
\definecolor{building}{RGB}{255, 200, 0}
\definecolor{barrier}{RGB}{255, 120, 50}
\definecolor{other}{RGB}{55, 90, 80}
\definecolor{pedestrian}{RGB}{255, 30, 30}
\definecolor{pole}{RGB}{255, 240, 150}
\definecolor{road}{RGB}{255, 0, 255}
\definecolor{ground}{RGB}{175, 0, 75}
\definecolor{sidewalk}{RGB}{75, 0, 75}
\definecolor{vegetation}{RGB}{0, 175, 0}
\definecolor{vehicles}{RGB}{100, 150, 245}

\begin{table*}[p]{
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}
{\normalsize
\begin{tabular}{c|cccccccccccc|c}
\hline
\multirow{3}{*}{} & \multicolumn{12}{c|}{Class IoU} & \multirow{3}{*}{IoU} \\ \cline{2-13}
 & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textcolor{building}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{barrier}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{other}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{pedestrian}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{pole}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{road}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{ground}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{sidewalk}{$\blacksquare$}} & \multicolumn{1}{c}{\textcolor{vegetation}{$\blacksquare$}} & \multicolumn{1}{c|}{\textcolor{Vehicles}{$\blacksquare$}} &  \\ 
 & \multicolumn{1}{c|}{\multirow{1}{*}{mIoU}} & Free & Building & Barrier & Other & Pedestrian & Pole & Road & Ground & Sidewalk & Vegetation &  vehicles\\ \hline
w/o Diffusion & \multicolumn{1}{c|}{40.09} & 96.15 & 28.55 & \textbf{4.20} & 7.91 & 26.62 & 39.72 &  84.92 &  7.83 &  65.97 & 31.76 & 47.33 & 78.81 \\
Discrete Diffusion & \multicolumn{1}{c|}{\textbf{45.09}} & 96.00 & \textbf{31.92} & 2.38 & \textbf{23.95} & \textbf{47.21} & \textbf{42.86} & 85.30 & \textbf{9.43} & \textbf{66.79} & \textbf{34.38} & \textbf{55.78} & 78.54 \\ \hline
\end{tabular}
}
}
\caption{Our semantic scene completion results on test set of CarlaSC. The discriminative learning result with the diffusion model architecture is denoted as `w/o Diffusion'. %To compare meaningful results, 
Values with a difference equal or greater than 0.5\%p are bold.}
\label{tab:ours}
\end{table*}
